Reproducing NevIR: Negation in Neural Information Retrieval

Negation is a fundamental aspect of human communication, yet it remains a challenge for Language Models (LMs) in Information Retrieval (IR). Despite the heavy reliance of modern neural IR systems on LMs, little attention has been given to their handling of negation. In this study, we reproduce and extend the findings of NevIR, a benchmark study that revealed most IR models perform at or below the level of random ranking when dealing with negation. We replicate NevIR's original experiments and evaluate newly developed state-of-the-art IR models. Our findings show that a recently emerging category-listwise Large Language Model (LLM) re-rankers-outperforms other models but still underperforms human performance. Additionally, we leverage ExcluIR, a benchmark dataset designed for exclusionary queries with extensive negation, to assess the generalisability of negation understanding. Our findings suggest that fine-tuning on one dataset does not reliably improve performance on the other, indicating notable differences in their data distributions. Furthermore, we observe that only cross-encoders and listwise LLM re-rankers achieve reasonable performance across both negation tasks.

==> sections/old_discussion.tex <==

\section{Discussion and Conclusion}

\coen{structure: we now have claim -> what we thing (and possibly extensions) for every claim. do we want to keep this or convert to story}

In this section, the findings of our research are discussed. We also discuss wether or not these findings support the claims the authors make.

\subsubsection*{Claim 1:} The researchers provide a benchmark (dataset), together with a metric for Negation Evaluation in Information Retrieval to  fill the literature gap of negation in IR models. \\

A shortcoming of the paper is its reliance on pairwise accuracy, a non-standard IR metric, which limits its broader applicability to IR tasks. The metric  tests whether a model can differentiate between two specific documents, offering insights into LMs’ handling of negation but limited implications for broader IR tasks. Thus, while the metric offers some insights in IR performance, the study provides more value for NLP negation research than for IR system evaluation.
Another limitation of the paper is its lack of a baseline to evaluate the model’s general performance on the data distribution. To assess performance on the negation task, the authors included a random baseline (25\%). However, we argue that an additional baseline—evaluating the model’s overall performance on this data distribution—should have been included. This would help clarify whether the poor performance stems from the model’s difficulty with ranking documents involving negation or from an out-of-distribution (OOD) effect.

Future research should focus on developing a more effective benchmark for negation performance to address the current limitations. One potential solution is to construct a negation dataset from an existing IR dataset on which models are trained, such as MS MARCO, which would mitigate the OOD issue. This benchmark could then be evaluated using standard IR metrics like MRR@10. When creating the dataset, it is crucial to include diverse examples of negation to ensure the model’s ability to generalize negation comprehension.

\subsubsection*{Claim 2:} The researchers find that nearly all IR systems ignore the negation, stating the relevance of this research. \\

In our reproduction of the benchmarking study, while some scores slightly deviate from the authors and some models could not be evaluated due to dependency issues, we verified this claim. Furthermore, in line with the original paper, we find that nearly all IR systems ignore the negation, stating the relevance of this research.

\subsubsection*{Extending Research on This Claim}  
In our extension of this claim, we evaluated new SOTA models and observed improvements across all tested categories. Notably, the GritLM model in the bi-encoder category demonstrated significant improvements, achieving performance comparable to many cross-encoders. Similarly, the Jina-reranker-v2-base-multilingual in the cross-encoder category also had quite impressive performance, with results close to the RankGPT-4o-mini model, which is even more notable given its relatively small size. 

Despite these improvements, these best models still fall far short of achieving human-level performance. These findings support the claim that nearly all neural IR models fail to adequately handle negation and highlight that understanding negation continues to be a significant challenge for neural IR systems.

\subsubsection*{Claim 3:} The researchers show that continued fine-tuning of IR models on negation data provides some gains on NevIR, but still leaves significant room to improve (while also slightly hurting performance on traditional benchmarks such as MS MARCO). \\

In our reproduction of the finetuning experiments, we find the same results as the authors and verified this claim. With finetuning, models increase in performance on NevIR, while decrease in performance on IR tasks.

\subsubsection*{Extending research on this claim}: 
When looking into a more balanced way of finetuning for IR purposes, our findings indicate that fine-tuning on a merged dataset combining NevIR and MS MARCO led to slightly different results across various models. Although these results show some fluctuation, we argue that carefully selecting the best model based on performance across both development sets can lead to more stable results, ensuring better performance on both the targeted and original tasks. We do note that this preliminary result is only marginal and needs to be explored further.

Including more training data with additional and diverse examples from the ExcluIR dataset  did not improve the IR models' ability to handle negation effectively. This suggests that the model is not adequately utilizing the additional negation information from the ExcluIR data. This implies that the NevIR dataset may not be sufficiently diverse to cover all forms of negation, such as exclusion. This hypothesis is supported by the fact that the NevIR training set only has 1896 samples, which could be insufficient to properly cover the entire spectrum of negation. Furthermore, the observed performance improvement on the NevIR dataset when fine-tuned exclusively on it may be more attributable to the model learning the underlying data distribution rather than truly understanding negation. 

For investigating the generalization of negation comprehension learned from the NevIR dataset, we evaluated the models fine-tuned on NevIR on ExcluIR. The results showed that only the cross-encoder model demonstrated effective transfer of negation comprehension to this new setting. This is likely due to the cross-encoder’s large model size and its ability to combine query and documents into the most expressive representation among the different model categories. This suggest that the cross-encoder is the only model that meaningfully represents negation in a way that generalizes across different data distributions and contexts. Furthermore, this finding reinforces our hypothesis that the bi-encoder and late interaction models have "solved" the task by learning patterns unrelated to actual negation, such as other shortcuts or heuristics, which allow them to perform well on the NevIR task without truly understanding negation.

To gain a deeper understanding of what these models then actually learn during finetuning,  a preliminary qualitative analysis was conducted with ColBERTv1. These observations suggested that while the model improves at recognizing straightforward negations through fine-tuning, it still faces challenges when dealing with more complex, context-sensitive negation. This could also explain the poor performance of the finetuned models on ExcluIR, as exclusion is often more implicit and context-sensitive negation. Future work should focus on a deeper qualitative analysis and quantification of the proposed hypotheses. 

\subsection{Environmental impact}  
\coen{rewrite after experiments AND MENTION gpt-4o impact in water?}
The reproducible experiments totaled approximately 49 GPU hours, see \autoref{app:gpu_hours} for a detailed calculation. Additional exploratory runs and repeated experiments increased the cumulative computational time to approximately 100 hours. All experiments were conducted on NVIDIA H100 PCIe GPUs (TDP of 350W) using the Snellius supercomputer, which has a carbon efficiency of 0.421 kgCO$_2$eq/kWh.  

We could not find a calculator for the used H100 gpu's, so we approximated the impact by using the MachineLearning Impact calculator with A100 PCIe 40/80GB GPU \cite{lacoste2019quantifying}. Total emissions are estimated post hoc to be approximately \textbf{6.75 kgCO$_2$eq}. Estimations were conducted using the \href{https://mlco2.github.io/impact#compute}{MachineLearning Impact calculator} presented in \cite{lacoste2019quantifying}.This estimation includes both the power consumption of the GPUs and the energy efficiency of the hardware infrastructure.

==> tables/table3.tex <==
\begin{table}[tbp]
  \caption{Model performance in accuracy for NevIR and ExcluIR, fine-tuned on different negation datasets.}
  \label{tab:merge_test_performance}
  \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{cclcc}
    \toprule
    Type & Model Name & Finetune & NevIR & ExcluIR \\
    \midrule
    Bi-Encoder & multi-qa-mpnet & None & 11.1\% & 71.3\% \\
    & & NevIR & 50.6\% & 51.2\%\\
    & & ExcluIR & 9.5\% & 93.3\%\\
    & & ExcluIR + NevIR & 51.9\% & 94.1\% \\
    \midrule
    Late Interaction & ColBERTv1 & None & 19.9\% & 66.8\% \\
    &   & NevIR & 47.0\% & 64.5\% \\
    &   & ExcluIR & 12.7\% & 90.7\% \\
    &   & ExcluIR + NevIR & 40.6\% & 90.5\% \\
    % & ColBERTv1 & MSMarco + NevIR & 46.1\% & - \\
    \midrule
    Cross-Encoder & MonoT5 base & None & 34.9\% & 68.37\% \\
    & & NevIR & 73.4\% & 77.5\% \\
    &  & ExcluIR & 45.2\% & 90.1\% \\
    &  & ExcluIR + NevIR & 71.8\% & 93.0\% \\
    % & MonoT5 base & MSMarco + NevIR & 71.7\% & - \\
    \midrule
    Listwise LLM & Mistral-7B-Instruct & None & 38.66\% & 93.93\% \\
    &  & NevIR & 73.33\% & 89.31\% \\
    &  & ExcluIR & 23.5\% & 96.8\% \\
    &  & ExcluIR + NevIR & 72.9\% & 96.8\% \\
    \bottomrule
  \end{tabular}
  }
\end{table}
% \begin{table}[htbp]
%   \caption{Model performance in accuracy for NevIR and ExcluIR, fine-tuned on different negation datasets.}
%   \label{tab:merge_test_performance}
%   \resizebox{0.5\textwidth}{!}{
%   \begin{tabular}{cclcc}
%     \toprule
%     Type & Model Name & Finetune Set & NevIR Score & ExcluIR Score \\
%     \midrule
%     Bi-Encoder & multi-qa-mpnet-base-dot-v1 & None & 11.1\% & 71.3\% \\
%     & multi-qa-mpnet-base-dot-v1 & NevIR & 50.6\% & 51.2\%\\
%     & multi-qa-mpnet-base-dot-v1 & ExcluIR & 9.5\% & 93.3\%\\
%     & multi-qa-mpnet-base-dot-v1 & ExcluIR + NevIR & 51.9\% & 94.1\% \\
%     \midrule
%     Late Interaction & ColBERTv1 & None & 19.9\% & 66.8\% \\
%     & ColBERTv1 & NevIR & 47.0\% & 64.5\% \\
%     & ColBERTv1 & ExcluIR & 12.7\% & 90.7\% \\
%     & ColBERTv1 & ExcluIR + NevIR & 40.6\% & 90.5\% \\
%     % & ColBERTv1 & MSMarco + NevIR & 46.1\% & - \\
%     \midrule
%     Cross-Encoder & MonoT5 base & None & 34.9\% & 68.37\% \\
%     & MonoT5 base & NevIR & 73.4\% & 77.5\% \\
%     & MonoT5 base & ExcluIR & 45.2\% & 90.1\% \\
%     & MonoT5 base & ExcluIR + NevIR & 71.8\% & 93.0\% \\
%     % & MonoT5 base & MSMarco + NevIR & 71.7\% & - \\
%     \midrule
%     Listwise LLM & Mistral-7B-Instruct-v0.3 & None & 38.66\% & 93.93\% \\
%     & Mistral-7B-Instruct-v0.3 & NevIR & 73.33\% & 89.31\% \\
%     & Mistral-7B-Instruct-v0.3 & ExcluIR & 23.5\% & 96.8\% \\
%     & Mistral-7B-Instruct-v0.3 & ExcluIR + NevIR & 72.9\% & 96.8\% \\
%     \bottomrule
%   \end{tabular}
%   }
% \end{table}

% \begin{table*}[h]
%   \caption{Model Performance with finetune set}
%   \label{tab:merge_test_performance}
%   \begin{tabular}{cclcc}
%     \toprule
%     Type & Model Name & Finetune Set & NevIR Score & ExcluIR Score \\
%     \midrule
%     Bi-Encoder & multi-qa-mpnet-base-dot-v1 & None & 11.1\% & 27.4\% \\
%     & multi-qa-mpnet-base-dot-v1 & NevIR & 52.1\% & 28.9\% \\
%     & multi-qa-mpnet-base-dot-v1 & ExcluIR & 7.23\% & 47.9\% \\
%     & multi-qa-mpnet-base-dot-v1 & ExcluIR + NevIR & 50.0\% & 44.8\% \\
%     % & multi-qa-mpnet-base-dot-v1 & MSMarco + NevIR & 50.1\% & - \\
%     \midrule
%     Late Interaction & ColBERTv1 & None & 19.9\% & 26.0\% \\
%     & ColBERTv1 & NevIR & 47.0\% & 25.5\% \\
%     & ColBERTv1 & ExcluIR & 10.0\% & 45.5\% \\
%     & ColBERTv1 & ExcluIR + NevIR & 38.2\% & 46.0\% \\
    
    
%     % & ColBERTv1 & MSMarco + NevIR & 46.1\% & - \\
%     \midrule
%     Cross-Encoder & MonoT5 base & None & 34.9\% & 23.8\% \\
%     & MonoT5 base & NevIR & 72.7\% & 35.9\% \\
%     & MonoT5 base & ExcluIR & 43.0\% & 50.3\% \\
%     & MonoT5 base & ExcluIR + NevIR & 71.6\% & 50.5\% \\
    
%     % & MonoT5 base & MSMarco + NevIR & 71.7\% & - \\
%     \midrule
%     Listwise LLM & \\
%     \\
%     \\
%     \\
%     \bottomrule
%   \end{tabular}
% \end{table*}
